Understanding Physical Dynamics with Counterfactual World Modeling

The ability to understand physical dynamics is critical for agents to act in the world. Here, we use Counterfactual World Modeling (CWM) to extract vision structures for dynamics understanding. CWM uses a temporally-factored masking policy for masked prediction of video data without annotations. This policy enables highly effective "counterfactual prompting" of the predictor, allowing a spectrum of visual structures to be extracted from a single pre-trained predictor without finetuning on annotated datasets. We demonstrate that these structures are useful for physical dynamics understanding, allowing CWM to achieve the state-of-the-art performance on the Physion benchmark.

==> algorithmtex/cosine_flow.tex <==
%\renewcommand{\thealgorithm}{}
\begin{algorithm}[t]
\scriptsize
\newcommand{\AlignedComment}[1]{\hfill\makebox[3.3cm][l]{$\triangleright$ \scriptsize\gray{#1}}} % Adjust the width as needed
\captionsetup{font=scriptsize}
\caption{Efficient optical flow for ViT embeddings}
% % \hspace*{\algorithmicindent} \textbf{Input}: \\
% %  \hspace*{\algorithmicindent} \textbf{Output}:
\begin{algorithmic}[1] % The number indicates line numbering interval


\Procedure{efficient\_optical\_flow}{$e1, e2$}

    \State $X \gets \Call{CosineSimilarity}{e1, e2}$
    \AlignedComment{compute similarity matrix}    
    \State $Y \gets \Call{argmax}{X}$
    \AlignedComment{argmax to find most similar}
    \State $d \gets x_2 - Y$
    \AlignedComment{displacement from $x_1$ to $x_2$}

    \State $Flow \gets \Call{AssignDisplacement}{d}$
    \AlignedComment{construct flow map}    

    \State \textbf{return} $Flow$
\EndProcedure

\end{algorithmic}
\label{algorithm:cosine_flow}
\end{algorithm}


==> algorithmtex/keypoint.tex <==
\renewcommand{\thealgorithm}{}
\newcommand{\AlignedComment}[1]{\hfill\makebox[3.3cm][l]{$\triangleright$ \scriptsize\gray{#1}}} % Adjust the width as needed
\begin{algorithm}[H]
\scriptsize
\captionsetup{font=scriptsize}
\caption{Extract keypoints}
% \hspace*{\algorithmicindent} \textbf{Input}: \\
%  \hspace*{\algorithmicindent} \textbf{Output}:
\begin{algorithmic}[1] % The number indicates line numbering interval

\Procedure{extract\_keypoint}{$x_1, x_2$} 
    
    \State $K \gets \varnothing$ \AlignedComment{K represents a set of keypoints}
    \State $a \gets \Call{zeros\_like}{x_1}$ \AlignedComment{initialize action as empty frame}
    \For{$ 1$ \textbf{to} $iter$} \AlignedComment{each iteration adds 1 keypoint}
        \State $\tilde{x} \gets \Psi(x_1, a)$ \AlignedComment{predicting next frame}
        \State $err \gets \Call{mse}{\tilde{x}, x_2}$ \AlignedComment{compute reconstruction error}
        \State $(i,j) \gets \Call{argmax\_2d}{err}$ \AlignedComment{select (i,j) with max error}
        \State $K \gets K \cup (i,j)$ \AlignedComment{add to the set of keypoints}
        \State $p \gets \Call{zeros\_like}{x}$ \AlignedComment{initialize a probability map}
        \State $p[i, j] \gets 1$ \AlignedComment{1 at the keypoint location}
        
        \State $a \gets \Call{Sample}{x_2, p, 1, 0}$ \AlignedComment{equivalent to $a[i, j]\gets x_2[i, j]$}
    \EndFor
    \State \Return $K$ \AlignedComment{list of keypoint locations}
\EndProcedure

\end{algorithmic}
\label{algorithm:keypoint}
\end{algorithm}


==> algorithmtex/keypoints_v2.tex <==

\begin{wrapfigure}{r}{0.42\textwidth} % 'l' for left and '0.5\textwidth' for the width of the wrap figure
\vspace{-1.6cm}
    \begin{minipage}{0.42\textwidth}
        \begin{algorithm}[H]
        \scriptsize
        \captionsetup{font=scriptsize}
        
        \caption{Keypoint extraction}
            \begin{algorithmic}[1]
            
               \Procedure{keypoint}{$x_1, x_2$} 
    
                \State $K \gets \varnothing$ 
                \State $a \gets \Call{zeros\_like}{x_1}$ 
                \For{$ 1$ \textbf{to} $iter$} 
                    \State $\tilde{x} \gets \Psi(x_1, a)$ 
                    \State $err \gets \Call{mse}{\tilde{x}, x_2}$ 
                    \State $(i,j) \gets \Call{argmax\_2d}{err}$ 
                    \State $K \gets K \cup (i,j)$ 
                    \State $p \gets \Call{zeros\_like}{x}$ 
                    \State $p[i, j] \gets 1$ 
                    
                    \State $a \gets \Call{Sample}{x_2, p, 1, 0}$ 
                \EndFor
                \State \Return $K$ 
            \EndProcedure
            \end{algorithmic}
        \label{algorithm:keypoint}
        
        \end{algorithm}
        \vspace{-1.2cm}
    \end{minipage}
    
    
\end{wrapfigure}



==> algorithmtex/optical_flow.tex <==
\renewcommand{\thealgorithm}{}
\begin{algorithm}[H]
\scriptsize
\newcommand{\AlignedComment}[1]{\hfill\makebox[3.3cm][l]{$\triangleright$ \scriptsize\gray{#1}}} % Adjust the width as needed
\captionsetup{font=scriptsize}
\caption{Extract optical flow at location $(i, j)$}
% % \hspace*{\algorithmicindent} \textbf{Input}: \\
% %  \hspace*{\algorithmicindent} \textbf{Output}:
\begin{algorithmic}[1] % The number indicates line numbering interval


\Procedure{prompt\_optical\_flow}{$x_1$, $x_2$} 
    
    \State  $\bar{X} \gets \varnothing$
    \AlignedComment{init a list for predictions}
    \State  $p \gets \Call{ones\_like}{x_2}$
    \AlignedComment{uniform sampling distribution}
    \State  $p \gets p_k / \sum_{k} p_k$
    \AlignedComment{normalization}
    
    \For{$ 1$ \textbf{to} $iter$} 
    \AlignedComment{loop over mask samples}
    
        \State $a = \Call{sample}{x_2, p, n, 0}$
        \AlignedComment{sample actions with $x_2$ patches}
        \State $\bar{x}_1 \gets x_1 + \delta_i$
        \AlignedComment{perturb frame 1}
%        \State  $X \gets X \oplus \Psi(x_1, a)$
        \State  $\bar{X} \gets \bar{X} \oplus \Psi(\bar{x}_1, a)$
        \AlignedComment{store the perturbed prediction}
    \EndFor

    \State  $\bar{\delta} \gets |\Call{mean}{{\bar{X}}}-x_2|$
    \AlignedComment{compute perturbation response}

    \State  $i', j' \gets \Call{argmax\_2d}{\bar{\delta}}$  
    \AlignedComment{locate the perturbation in $x_2$}
    \State $flow \gets (i'\!-\!i, j'\!-\!j)$
    \AlignedComment{flow is the displacement}
    \State \Return $flow$
    \AlignedComment{flow for location $i$}
\EndProcedure

\end{algorithmic}
\label{algorithm:flow}
\end{algorithm}


==> algorithmtex/optical_flow_v2.tex <==

\begin{wrapfigure}{r}{0.42\textwidth} % 'l' for left and '0.5\textwidth' for the width of the wrap figure
\vspace{-1.6cm}
    \begin{minipage}{0.42\textwidth}
        \begin{algorithm}[H]
        \scriptsize
        \captionsetup{font=scriptsize}
        
        \caption{Flow extraction at ($i$, $j$)}
            \begin{algorithmic}[1]
            
               \Procedure{flow}{$x_1$, $x_2$} 
    
                \State  \textit{R} \gets \varnothing $
                
                \State  $p \gets \Call{ones\_like}{x_2}$
                \State  $p \gets p_k / \sum_{k} p_k$
    
                
                \For{$ 1$ \textbf{to} $iter$} 
   
                    \State $a = \Call{sample}{x_2, p, n, 0}$
                    % \State $\bar{x}_1 \gets x_1 + \delta_i$
                    \State  $\tilde{x}_2^p \gets \Psi(x_1 + \delta_{ij}, a)$
                    \State  $\tilde{x}_2 \gets \Psi(x_1, a)$
                    \State $\textit{R} \gets \textit{R} \oplus |\tilde{x}_2^p - \tilde{x}_2 |$
    
                \EndFor
            
                \State  $\bar{\delta} \gets \Call{mean}{R}$
                \State  $i', j' \gets \Call{argmax\_2d}{\bar{\delta}}$  
                \State $flow \gets (i'\!-\!i, j'\!-\!j)$
                \State \Return $flow$
            \EndProcedure

            \end{algorithmic}
        \label{algorithm:flow}
        
        \end{algorithm}
        \vspace{-1.2cm}
    \end{minipage}
    
    
\end{wrapfigure}



==> algorithmtex/sampling_operator.tex <==
\begin{algorithm}[t]
\newcommand{\AlignedComment}[1]{\hfill\makebox[3.cm][l]{$\triangleright$ \scriptsize\gray{#1}}} % Adjust the width as needed
\scriptsize
\captionsetup{font=scriptsize}
\caption{Sampling actions}
% \hspace*{\algorithmicindent} \textbf{Input}: $x \in \mathbb{R}^{3 \times H \times W}, \, p \in  \mathbb{R}^{H' \times W'}\, n, c \in \mathbb{Z}^{\ge 0}$\\
%  \hspace*{\algorithmicindent} \textbf{Output}: $c \in \mathbb{R}^{3 \times H \times W}$ 
\begin{algorithmic}[1]

\Function{sample}{$x$, $p$, $n$, $r$} 
    % \State $a \gets \Call{zero\_like}{x}$ \AlignedComment{initialize an empty action}
    % \State $\epsilon_1, \epsilon_2 \sim \Call{Uniform}{-r, r}$ \AlignedComment{sample a location offset}
    % \For{$ 1$ \textbf{to} $n$} \AlignedComment{iterate to sample n patches}
    % \State $(i, j) \sim \Call{multinomial}{p, 1}$ \AlignedComment{sample a patch location}
    % \State $a[i\!+\!\epsilon_1, j\!+\!\epsilon_2] \gets x[i, j]$ \AlignedComment{copy the patch content}
    % \EndFor
    % \State \Return $a$ \AlignedComment{$a \!\in\! \mathbb{R}^{3 \times H \times W}$}
    \State $a \gets \Call{zero\_like}{x}$ 
    \State $\epsilon_1, \epsilon_2 \sim \Call{Uniform}{-r, r}$ 
    \For{$ 1$ \textbf{to} $n$} 
    \State $(i, j) \sim \Call{multinomial}{p, 1}$ 
    \State $a[i\!+\!\epsilon_1, j\!+\!\epsilon_2] \gets x[i, j]$ 
    \EndFor
    \State \Return $a$ 
\EndFunction

\end{algorithmic}

\label{algorithm:operator}
% \vspace{-0.1cm}
\end{algorithm}



==> algorithmtex/sampling_operator_v2.tex <==

\begin{wrapfigure}{r}{0.37\textwidth} % 'l' for left and '0.5\textwidth' for the width of the wrap figure
\vspace{-1.6cm}
    \begin{minipage}{0.37\textwidth}
        \begin{algorithm}[H]
        \scriptsize
        \captionsetup{font=scriptsize}
        
        \caption{Sampling actions}
            \begin{algorithmic}[1]
            
                \Function{sample}{$x$, $p$, $n$, $r$} 
                    \State $a \gets \Call{zero\_like}{x}$ 
                    \For{$ 1$ \textbf{to} $n$} 
                    \State $(i, j) \sim \Call{multinomial}{p, 1}$ 
                    \State $\epsilon_1, \epsilon_2 \sim \Call{Uniform}{-r, r}$ 
                    \State $a[i\!+\!\epsilon_1, j\!+\!\epsilon_2] \gets x[i, j]$ 
                    \EndFor
                    \State \Return $a$ 
                \EndFunction
            \end{algorithmic}
        \label{algorithm:operator}
        
        \end{algorithm}
        \vspace{-1.5cm}
    \end{minipage}
    
    
\end{wrapfigure}



==> algorithmtex/segmentation.tex <==
\renewcommand{\thealgorithm}{}
\newcommand{\AlignedComment}[1]{\hfill\makebox[3.4cm][l]{$\triangleright$ \scriptsize\gray{#1}}} % Adjust the width as needed
\begin{algorithm}[H]
\scriptsize
\captionsetup{font=scriptsize}
\caption{Extract Spelke object segment at location $(i, j)$}
\begin{algorithmic}[1] % The number indicates line numbering interval


\Procedure{prompt\_segment}{$x$} 
    
    \State $p \gets \Call{zeros\_like}{x}$  \AlignedComment{init probability distribution}
    \State $p[i, j] \gets 1$ \AlignedComment{set as 1 in the queried location}
    \State $n \gets 1$  \Comment{\gray{\footnotesize{start with sampling 1 patch in the action}}}
    \For{$ 1$ \textbf{to} $iter$}
    \State $a \gets \Call{Sample}{x, p, n, r}$ \AlignedComment{sample counterfaction motion}
    %\State $c_{stop} \gets \Call{Sample}{x, -p, n, 0}$ 
    \State $\tilde{x} \gets \Psi(x, a)$ \AlignedComment{predict next frame}
    \State $flow \gets \Call{Flow}{x, \tilde{x}}$ \AlignedComment{compute flow between $x$ and $\tilde{x}$}
    \State $seg \gets \Call{norm}{flow} > 0$ \AlignedComment{threshold flow magnitude}
    \State $p \gets p + seg$ \AlignedComment{update p for next iteration}
    \State  $p \gets p_k / \sum_{k} p_k$ \AlignedComment{normalization}
    
    \State $n \gets n+1$ \Comment{\gray{\footnotesize{sample more patches in next iteration}}} 
    
    \EndFor
    \State \Return $seg$ \Comment{\gray{\footnotesize{binary segmentation map of shape $H\!\times\! W$}}}
\EndProcedure

\end{algorithmic}
\label{algorithm:segmentation}
\end{algorithm}


==> algorithmtex/segmentation_v2.tex <==

\begin{wrapfigure}{r}{0.42\textwidth} % 'l' for left and '0.5\textwidth' for the width of the wrap figure
\vspace{-1.6cm}
    \begin{minipage}{0.42\textwidth}
        \begin{algorithm}[H]
        \scriptsize
        \captionsetup{font=scriptsize}
        
        \caption{Segment extraction at ($i$, $j$)}
            \begin{algorithmic}[1]
                \Procedure{segment}{$x$} 
    
                \State $p \gets \Call{zeros\_like}{x}$ 
                \State $p[i, j] \gets 1$
                \State $n \gets 1$  
                \For{$ 1$ \textbf{to} $iter$}
                \State $a \gets \Call{Sample}{x, p, n, r}$ 
                %\State $c_{stop} \gets \Call{Sample}{x, -p, n, 0}$ 
                \State $\tilde{x} \gets \Psi(x, a)$ 
                \State $flow \gets \Call{Flow}{x, \tilde{x}}$ 
                \State $seg \gets \Call{norm}{flow} > 0$ 
                \State $p \gets p + seg$ 
                \State  $p \gets p_k / \sum_{k} p_k$ 
                
                \State $n \gets n+1$ 
                
                \EndFor
                \State \Return $seg$
            \EndProcedure

               

            \end{algorithmic}
        \label{algorithm:segment}
        
        \end{algorithm}
        \vspace{-1.2cm}
    \end{minipage}
    
    
\end{wrapfigure}



==> figtex/extracted_structures.tex <==
\begin{figure*}[t]
    \centering
    \includegraphics[width=0.98\linewidth]{figures/extracted_structures_copy.pdf}
    \caption{Zero-shot extraction of keypoints, optical flow, and segments by CWM.}
    \label{fig:extraction}
    \vspace{-0.4cm}
\end{figure*}

==> figtex/fig2_predictions.tex <==
\begin{figure}[t]
    \centering
    \includegraphics[width=0.98\linewidth]{figures/fig2-predictions-v4.png}
    \caption{A small number of visual patches exert meaningful control of scene dynamics. Each triplet shows the input image (left), an action constructed from the input image (middle), and the counterfactual prediction of the model (right). Each action is constructed by copying 2-3 patches from the input image. A red patch in the action is copied from the input image into the same location as its source. This prompts the predictor to simulate the appearance of holding an object fixed.  A green patch is copied from the input image, but into a different location at an offset from the source location. This simulates the appearance of an apparent object motion.}
    \label{fig:counterfactual}
    \vspace{-0.6cm}
\end{figure}

==> figtex/fig3-keypoint.tex <==
\begin{figure}[t]
    \centering
    
    \begin{minipage}{0.46\textwidth}
        \centering
        \includegraphics[width=\textwidth]{figures/fig3-keypoint-program-without-illustrator.pdf} % replace with your image
        \vspace{-0.8cm}
    \end{minipage}
    
    \begin{minipage}{0.46\textwidth}
        \centering
        \input{algorithmtex/keypoint}
    \end{minipage}\hfill
    
    \vspace{0.1cm}
    \begin{minipage}{0.46\textwidth}
        \centering
        \includegraphics[width=\textwidth]{figures/fig3-keypoint-results-without-illustrator.pdf} % replace with your image
    \end{minipage}
    
    \caption{\textbf{Counterfactual query for keypoints} The first panel and the algorithm describe an iterative procedures for extracting keypoints given an frame pair $x_1,x_2$ as input. Starting with an action with no visible patches, the algorithm selects a location with maximum reconstruction error as the keypoint. The keypoint patch is then added to the action in the next iteration, and this process iterates to extract multiple keypoints $K$. The last panel shows that with only 8 keypoints (1\% of the totalpatches), the predictor is capable of predicting the next frame and capturing dynamics well.}
    \label{fig:keypoint}
    \vspace{-0.6cm}
\end{figure}

==> figtex/fig4-flow.tex <==
\begin{figure}[t]
    \centering
    
    \begin{minipage}{0.3\textwidth}
        \centering
        \includegraphics[width=\textwidth]{figures/fig4-flow-program-without-illustrator.pdf} % replace with your image
        \vspace{-0.6cm}
        \label{fig:my_label}
    \end{minipage}
    
    
    \vspace{0.2cm}
    \begin{minipage}{0.3\textwidth}
        \centering
        \includegraphics[width=\textwidth]{figures/davis_flow_copy-without-illustrator.pdf} % replace with your image
    \end{minipage}
    
    \caption{\textbf{Counterfactual query for flow.} The first panel and algorithm describe a procedure for extracting optical flow at location $(i,j)$. Flow is obtained by perturbing the first frame of the image at a given location, propagating the perturbation through the CWM, and comparing the perturbed response to the original second frame. Qualitative examples of optical flow on the DAVIS dataset \cite{davis2017} are shown here.}
    \vspace{-0.6cm}
    \label{fig:flow}
\end{figure}

==> figtex/fig5-segmentation.tex <==
\begin{figure}[t]
    \centering
    
    \begin{minipage}{0.49\textwidth}
        \centering
        \includegraphics[width=\textwidth]{figures/fig5-segmentation-program-without-illustrator.pdf} % replace with your image
        \vspace{-0.6cm}
        \label{fig:my_label}
    \end{minipage}
    
    \begin{minipage}{0.46\textwidth}
        \centering
        \input{algorithmtex/segmentation}
    \end{minipage}\hfill
    
    \vspace{0.3cm}
    \begin{minipage}{0.46\textwidth}
        \centering
        \includegraphics[width=\textwidth]{figures/fig5-segmentation-results-without-illustrator.pdf} % replace with your image
        
        \label{fig:my_label}
    \end{minipage}
    
    \caption{\textbf{Counterfactual query for extracting Spelke object segment}. The first panel and the algorithm describe an iterative procedure for extract segmentation at location $(i, j)$ of a static image $x$. CWM segments objects by sampling a counterfactual motion at the pixel location, predicting the next frame, and grouping together parts of the image that move similarly to the counterfactual motion. The last panel shows qualitative segmentation results on COCO \cite{locatello2020object} images. Three segmentation masks are extracted and shown for each image.} 
    \label{fig:segmentation}
    \vspace{-0.5cm}
\end{figure}

==> figtex/flow_results_qulitative.tex <==
\begin{figure}[t]
    \centering
    \includegraphics[width=1.0\linewidth]{figures/flow_results.pdf}
    \caption{\textbf{Unsupervised optical flow results on DAVIS}.}
    \label{fig:flow_qualitative}
\end{figure}

==> figtex/masking_ratio.tex <==
\begin{figure}[t]
    \centering
    \includegraphics[width=0.98\linewidth]{figures/masking ratio ocp ocd.pdf}
    \caption{\textbf{Masking ratio}. The y-axes are object contact prediction and detection accuracy respectively. A high masking ratio (90\%) works well for both OCP and OCD task. } \todo{TODO: get the data points for masking ratio 0.5 - 0.7}
    \label{fig:masking_ratio}
\end{figure}

==> figtex/prompt_segmentation.tex <==
\begin{figure}[ht]
    \centering
    
    \begin{minipage}{0.49\textwidth}
        \centering
        \includegraphics[width=\textwidth]{figures/fig3-prompting-segmentation.pdf} % replace with your image
        
        \label{fig:my_label}
    \end{minipage}

    \begin{minipage}{0.43\textwidth}
        \centering
        \input{algorithmtex/segmentation}
    \end{minipage}\hfill
    
    \caption{Caption for the figure}
\end{figure}

==> figtex/rebuttal/counterfactual.tex <==
\begin{figure}[t]
    \centering
    \includegraphics[width=0.98\linewidth]{figures/rebuttal-figure-small.pdf}
    \vspace{-0.3cm}
    \caption{Temporally-factored masking policy of CWM enables much better structure extractions and counterfactual predictions.}
  \label{fig:structure}
  \vspace{-1cm}
\end{figure}



==> figtex/supp_jacobian_cosine_flow_comparison.tex <==

\begin{figure*}
  \centering
  \includegraphics[width=0.99\linewidth]{figures/jacobian_cosine_similarity_copy_without_illustrator.pdf}

  \caption{\label{first}\textbf{Comparison between the pertubation method and cosine approximation} We compare the full perturbation-based optical flow extraction algorithm introduced in the main paper against the cosine-similarity approximation given in Algorithm  \ref{algorithm:cosine_flow}. The fidelity of the approximation method is very close to the complete flow estimate, while benefiting from much lower computational complexity.} 
  
  \label{fig:supp_jacobians_cosine_comparison}
\end{figure*}


==> figtex/teaser.tex <==
\begin{figure}[!t]
  \centering
  \fbox{\rule{0pt}{1.8in} \rule{0.9\linewidth}{0pt}}
   %\includegraphics[width=0.8\linewidth]{egfigure.eps}

   \caption{Teaser figure}
   \label{fig:onecol}
\end{figure}

==> tabletex/ablation.tex <==
\begin{table}[t] 
    \centering
    \tiny
    % \begin{tabular}{cc}
        \begin{subtable}{0.45\linewidth}
            \centering
            \begin{tabular}{ccc}
                \midrule
                Mask ratio & OCP $\uparrow$ & OCD $\uparrow$ \\
                \midrule
                0.85 & 73.4 & 87.3 \\
                0.90 & \textbf{73.9} & 87.1  \\
                0.95 & 73.4 &  \textbf{87.9} \\
                0.99 & 72.6 & 85.4 \\
                \midrule
            \end{tabular}
            \subcaption{Mask ratio}
            \label{ablation:mask_ratio}
        \end{subtable} 
        \begin{subtable}{0.45\linewidth}
            \centering
            \begin{tabular}{ccc}
                \midrule
                \#frames & OCP $\uparrow$ & OCD $\uparrow$ \\
                \midrule
                1 & 70.6 & 80.8 \\
                2 & \textbf{73.9} & \textbf{87.1} \\
                4 & 68.7 & 77.7 \\
                \midrule
            \end{tabular}
            \subcaption{Context length}
            \label{ablation:context_length}
            \vspace{2mm}
        \end{subtable} 
        \begin{subtable}{0.45\linewidth}
            \centering
            \begin{tabular}{ccc}
                \midrule
                Patch size & OCP $\uparrow$ & OCD $\uparrow$ \\
                \midrule
                16 & 73.5 & \textbf{87.3} \\
                8 & \textbf{73.6} & 87.1 \\
                \midrule
            \end{tabular}
            \subcaption{Patch size}
            \label{ablation:patch_size}
            \vspace{2mm}
        \end{subtable} 
        \begin{subtable}{0.45\linewidth}
            \centering
            \begin{tabular}{ccc}
                \midrule
                epochs & OCP $\uparrow$ & OCD $\uparrow$ \\
                \midrule
                800 & \textbf{73.6} & 87.1\\ 
                3200 & 73.6 & \textbf{89.1} \\
                \midrule
            \end{tabular}
            \subcaption{Training schedule}
            \label{ablation:training_schedule}
            \vspace{2mm}
        \end{subtable} 
        
        \begin{subtable}{0.98\linewidth}
            \centering
            \begin{tabular}{ccccccc}
            \toprule
            \multicolumn{4}{c}{Input to the linear classifier} & \multicolumn{2}{c}{Metric} \\
            \cmidrule(lr){1-4} \cmidrule(lr){5-6}
            Feat. & Keyp. & Flow & Segm. & OCP $\uparrow$ & OCD $\uparrow$ \\
            \midrule
            \checkmark & \xmark & \xmark & \xmark & 73.6 & 89.1 \\
            \checkmark & \checkmark & \xmark  & \xmark & 74.4 & 89.1   \\
            \checkmark & \checkmark & \checkmark & \xmark & 75.5 & 88.5   \\
            \checkmark & \checkmark & \checkmark & \checkmark & 75.9 & 89.1  \\
            \bottomrule
            \end{tabular}
            \subcaption{Utility of different vision structures}
            \label{tab:intermediates_ablation}
        \end{subtable}
    
    % \end{tabular}
    \caption{\textbf{CWM ablation studies.} In this set of tables, we study the effect of different architectural choices, training conditions and demonstrate the utility of different vision structures extracted from CWM towards improving performance on Physion tasks. Refer Section~\ref{sec:ablations} for a detailed description of the results.}
    \label{table:ablation}
\end{table}




==> tabletex/physion_results_v2.tex <==
\begin{table}[t!]
  \centering
  \scriptsize
  \begin{tabular*}{.9\linewidth}{@{\extracolsep{\fill}}llllcc}
    \toprule
    method & training data & arch & param & OCP\,$\uparrow$ & OCD\,$\uparrow$  \\
    \midrule
    \multicolumn{6}{l}{\textcolor{gray}{\textit{supervised ground truth 3D particle-based model}}} \\
    \midrule
    \textcolor{gray}{SGNN} & \textcolor{gray}{Physion v1.5} & \textcolor{gray}{GNN} & \textcolor{gray}{23 M} & \textcolor{gray}{76.4} & \textcolor{gray}{98.8}  \\
    \midrule
    \multicolumn{6}{l}{\textit{video prediction models}} \\
    \midrule
    MCVD & K400+Ego4D  & UNet & 251 M & 63.4 & 80.8 \\ 
    R3M  & K400+Ego4D  & Res50 & 38 M & 67.6 & 78.1 \\
    FitVid  & K400+Ego4D  &VAE & 303 M & 64.3 & 59.5 \\
    TECO  & K600  & vq-gan & 160 M & 69.3 & 80.9 \\
    \midrule
    \multicolumn{6}{l}{\textit{self-supervised image representation models}} \\
     \midrule
    DINO  & IN-1K  & ViT-B & 86M & 72.1 & 85.4 \\
    DINOv2  & LVD-142M  & ViT-B & 86 M & 72.2 & 87.1 \\
    DINOv2  & LVD-142M  & ViT-L & 304 M & 72.2 & 85.5 \\
    DINOv2  & LVD-142M  & ViT-g & 1.1 B & 72.7 & 84.6\\
    MAE  & IN-1K  & ViT-B & 86 M & 72.6 & 81.6\\
    MAE  & IN-1K  & ViT-L & 304 M & 71.6 & 82.3 \\
    MAE  & IN-1K  & ViT-H & 632 M & 73.3 & 80.8 \\
    MAE  & IN-4.5M  & ViT-B & 86 M & 72.1 & 81.7 \\
    MAE  & IN-4.5M  & ViT-L & 304 M & 72.6 & 81.9 \\
    
    \midrule
    
    \multicolumn{6}{l}{\textit{self-supervised video representation models}} \\
     \midrule
    VideoMAE & K400  & ViT-B & 86 M & 72.1 & 85.7  \\
    % VideoMAE+ \cite{tong2022videomae} & K400 & \xmark & ViT-B & 86 M &  &  \\
    VideoMAE* & K400  & ViT-B & 86 M & 73.2 & 86.2  \\
    VideoMAE  & K400  & ViT-L & 304 M & 73.6 & 86.1 \\
    VideoMAE  & K400  & ViT-H & 632 M & 73.5 & 87.5 \\
    VideoMAEv2  & U-Hybrid  & ViT-g & 1.1B & 72.2 & 85.0 \\
    V-JEPA  & VideoMix2M & ViT-L & 304M & 73.4 & 87.0 \\
    \midrule
    \multicolumn{6}{l}{\textit{vision-language models}} \\
    \midrule
    GPT4-V   & - & - & - & 52.9 & 54.7 \\
    \midrule
    \midrule
    % CWM-feat & K400 & \xmark & ViT-B & 86 M & 73.6 & 89.1\\
    % CWM-feat & K400 & \xmark & ViT-L & 304 M & 74.6 & 88.6 \\
    CWM & K400 & ViT-B & 86 M & 75.9 & \textbf{89.1}\\
    CWM & K400  & ViT-L & 304 M & \textbf{76.1} & 88.7\\
    
    \bottomrule
  \end{tabular*}
  \vspace{0.2cm}
  \caption{\textbf{State-of-the-art accuracy on Physion v1.5}. We compare CWM to five classes of baseline methods across different architectures on the OCP and OCD tasks. We evaluate CWM with both features and extracted structures and find that it achieves state-of-the-art performance on these tasks. Original VideoMAE \cite{tong2022videomae} uses 16 input frames and a patch size of 16. We trained VideoMAE* with 3 input frames, a patch size of 8, and include extracted vision structures from the model for a strictly fair comparison with CWM.}
  
  % \caption{\textbf{Physion v1.5 results.} We compare CWM to multiple model classes and architecture types on the OCP and OCD tasks. We find that CWM achieves superior performance to competing baselines on both tasks and does particularly well on the harder variant that tests for reasoning about future physical events (i.e OCP). Additionally, we also find that CWM can surpass the best prior method just by using the backbone features -- CWM-feat (73.6) vs MAE (72.6). The vision structures extracted from CWM using it's prompting capability further improve the OCP score to 75.9, surpassing prior methods by significant margins on the OCP task.}
  \label{tab:main_results}
  \vspace{-1.0cm}
\end{table}

==> tabletex/segmentation_results.tex <==
\begin{table}[t]
  \centering
  \scriptsize
  \resizebox{\columnwidth}{!}{
    \captionsetup{justification=centering}
  \begin{tabular}{lc}
  % First Subtable

  \begin{subtable}[t]{0.4\linewidth}
  \centering
  \begin{tabular}{lc}
    \toprule
    Method & epe $\downarrow$ \\
    \midrule
    RAFT~\cite{teed2020raft} & \textbf{1.476} \\
    PWCNet~\cite{sun2018pwc} & 2.288 \\
    SPyNet~\cite{ranjan2017optical} & 4.162 \\
    \midrule
    CWM & 4.981 \\
    \bottomrule
  \end{tabular}
  \subcaption{Flow Results \\ on SPRING}
  \label{tab:flow_spring} 
  \end{subtable} &
  % Second Subtable
  \begin{subtable}[t]{0.58\linewidth}
  \centering
  \begin{tabular}{lcc}
    \toprule
   Method &  $\text{AP}^{\text{box}}$ $\uparrow$ & $\text{AP}^{\text{mask}}$ $\uparrow$  \\
    \midrule
    TokenCut \cite{wang2023tokencut}  & 3.0 & 2.4 \\
    FreeSOLO \cite{wang2022freesolo}  & 4.2 & 4.3 \\
    CutLER \cite{wang2023cut}  & \textbf{10.8} & \textbf{8.42 }\\
    \midrule
    CWM & 10.0 & 8.20 \\
    \bottomrule
  \end{tabular}
  \subcaption{Detection and segmentation on \\ COCO val2017}
  \label{tab:segmentation_ap}
  \end{subtable}
  \end{tabular}
  }
  \caption{To assess the quality of CWM's zero shot vision structures, we show quantitative comparisons to baseline methods in (a) optical flow estimation on the SPRING benchmark and b) object detection and segmentation on COCO val2017.} 
 
\end{table}


==> text/figure_list.tex <==
fig 1. overview figure
fig 2. counterfactual predictions of CWM 
fig 3. extracted structures of cwm (Keyp, flow segment)
fig 4. comparison between cwm & videomae (counterfactual, Keyp, flow segment)

tab 1: (a) flow, counterfactual, (b) segment

fig 5. physion task
tab 2: physion results





option 2:

fig 0: overview 
fig 1. method figure
fig 2. CWM: counterfactual predictions, Keyp, flow segment)


fig 3. physion task
tab 1: physion results

analysis:
fig 4. comparison between cwm & videomae (counterfactual, Keyp, flow segment)
tab 2: ablations
tab 3: (a) flow, counterfactual, (b) segment



suggestion 
1. In the method section, say there is no general definition of keypoints


2. Figure 2: 
(a) learning association with temporal factoring
(b) intervention via prompts (change the counterfactual prompt to prompts)

3. Make the text in the figure biggers
